Search for New Heavy Particles Decaying to Z^0 Z^0 -> eeee in p-pbar Collisions at sqrt(s) = 1.96 TeV

We report the results of a search for the anomalous production of a massive particle decaying to four electrons via two Z^0 bosons in 1.1 fb^{-1} of p-pbar collisions at sqrt(s)=1.96 TeV collected by the CDF II detector at Fermilab. We employ optimized electron identification criteria to maximize acceptance and efficiency. We estimate the backgrounds in the invariant mass range 500 - 1000 GeV/c^2 to be 0.028 +/- 0.009 (stat) +/- 0.011 (syst) events. We observe zero events in this search region. Assuming a Randall-Sundrum graviton production model, we set 95% CL limits on \sigma times BF(G -> Z^0 Z^0) < 4 - 6 pb, depending on the graviton mass.

==> Makefile <==
###############################################################################
#                                                        December 4, 2002
#
# Makefile for a sample CDF Note - Stefan Stonjek  <s.stonjek@physics.ox.ac.uk>
#                                  Martin Hennecke <hennecke@fnal.gov> 
#
###############################################################################

TARGET = prd

# DO NOT EDIT BELOW

graphics_eps := $(wildcard *.eps)
graphics_pdf := $(patsubst %.eps,%.pdf,$(wildcard *.eps))


ps: $(TARGET).ps

pdf: $(TARGET).pdf

#$(TARGET).pdf: $(TARGET).tex $(wildcard */*.tex) $(graphics_eps)

$(TARGET).pdf: $(TARGET).tex $(wildcard */*.tex) $(graphics_pdf)
	pdflatex $(TARGET).tex && pdflatex $(TARGET).tex && thumbpdf $(TARGET) && pdflatex $(TARGET).tex

$(TARGET).dvi: $(TARGET).tex $(wildcard */*.tex) $(graphics_eps)
	latex $(TARGET).tex; latex $(TARGET).tex
$(TARGET).ps: $(TARGET).dvi
	dvips $(TARGET).dvi -o 

%.pdf: %.eps
	epstopdf $< 

$(PUBTARGET).pdf: $(PUBTARGET).tex $(wildcard */*.tex) $(graphics_pdf)
	pdflatex $(PUBTARGET).tex && pdflatex $(PUBTARGET).tex && thumbpdf $(PUBTARGET) && pdflatex $(PUBTARGET).tex


.PHONY: clean
clean:
	rm -r -f $(TARGET).aux $(TARGET).dvi $(TARGET).log $(TARGET).out $(TARGET).pdf \
	$(TARGET).ps $(TARGET).toc $(TARGET).tof thumb*.* *~ $(graphics_pdf)


==> xloosecem_pub.tex <==
\mbox{
\begin{tabular}{|c|c|c|}
\hline
Selection Criteria &  Trigger (CEM) & Minimal (CEM)\\
\hline
\hline
$E_T$(GeV)		& $\geq 20$                       	& $\geq 5$ \\
$|$Track $z_0|$ (cm) 	& $< 60 $ 				& $ < 60 $ \\
Had/EM       		& $< 0.055 + (0.00045 \times E)$  	&  $< 0.055 + (0.00045 \times E)$ \\
Isolation   		& $< 0.2 $                       	& $ < 0.2  $ \\
LshrTrk 		& $< 0.4 $ 				&  \\
Track $p_T$ (GeV/c) 	& $\geq 10 $ 				&  \\

%COT Axial Segments 	& $\geq 3 $ 				&  \\
%COT Stereo Segments 	& $\geq 2 $ 				&  \\
%Conversion		& $\neq 1 $ 				&  \\
%$E/p$ 			& $ \leq 2.0$ if $\pt < 50 GeV/c$ 	&  \\
%CES $\Delta z$ (cm) 	& $< 3.0 $ 				&  \\
%CES $\Delta x \times q$ & $-3.0 < \Delta x \times q < 1.5$ 	&  \\
%CES StripChi2 		& $< 10.0 $ 				&  \\
\hline

\end{tabular}
}


==> xloosepem_pub.tex <==
\mbox{
\begin{tabular}{|c|c|}
\hline
Selection Criteria & Minimal (PEM)\\
\hline
\hline
$E_T$(GeV)	      	& $\geq 5$ \\
Had/EM       		& $< 0.05$\\
Isolation   		& $< 0.2 $  \\
$|\eta_{\mathrm{det}}|$                & $< 2.5$ \\
%COT Axial Segments 	& $\geq 3 $ 				&  \\
%COT Stereo Segments 	& $\geq 2 $ 				&  \\
%Conversion		& $\neq 1 $ 				&  \\
%$E/p$ 			& $ \leq 2.0$ if $\pt < 50 GeV/c$ 	&  \\
%CES $\Delta z$ (cm) 	& $< 3.0 $ 				&  \\
%CES $\Delta x \times q$ & $-3.0 < \Delta x \times q < 1.5$ 	&  \\
%CES StripChi2 		& $< 10.0 $ 				&  \\
\hline

\end{tabular}
}

